Learning Multi-Aspect Item Palette: A Semantic Tokenization Framework for Generative Recommendation

Traditional recommendation models often rely on unique item identifiers (IDs) to distinguish between items, which can hinder their ability to effectively leverage item content information and generalize to long-tailed or cold-start items. Recently, semantic tokenization has been proposed as a promising solution that aims to tokenize each item's semantic representation into a sequence of discrete tokens. These semantic tokens have become fundamental in training generative recommendation models. However, existing methods typically rely on RQ-VAE, a residual vector quantizer, for semantic tokenization. This reliance introduces several key limitations, including challenges in embedding extraction, hierarchical coarse-to-fine quantization, and training stability. To address these issues, we introduce LAMIA, a novel approach for multi-aspect semantic tokenization. Unlike RQ-VAE, which uses a single embedding, LAMIA learns an ``item palette''--a collection of independent and semantically parallel embeddings that capture multiple aspects of items. Additionally, LAMIA enhances the semantic encoders through domain-specific tuning using text-based reconstruction tasks, resulting in more representative item palette embeddings. We have conducted extensive experiments to validate the effectiveness of the LAMIA framework across various recommendation tasks and datasets. Our results demonstrate significant improvements in recommendation accuracy over existing methods. To facilitate reproducible research, we will release the source code, data, and configurations.

==> Content/Figures/CodeTree.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.8\linewidth]{Assets/Figures/CodeTree.pdf}
    \caption{Code tree used in conditional beam search.}
    \label{fig:codetree}
\end{figure}


==> Content/Figures/Identifier.tex <==
\begin{figure}[]
    \centering
    \includegraphics[width=\linewidth]{Assets/Figures/Identifier}
    \caption{Comparison between conventional unique identifiers (in light green) and semantic identifiers (in light purple). For simplicity, each semantic identifier in this illustration consists of only two tokens.}
    \label{fig:identifier}
\end{figure}


==> Content/Figures/Paradigm.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{Assets/Figures/Paradigm.pdf}
    \caption{Comparison of the existing semantic tokenization pipeline (embedder → quantizer → recommender) with our proposed pipeline (tokenizer → clusterer → recommender).
    %Comparison between existing semantic tokenization pipeline, i.e., embedder -- quantizer -- recommender, with our proposed pipeline (below), i.e., tokenizer -- clusterer -- recommender.
    }
    \label{fig:paradigm}
\end{figure}


==> Content/Figures/Scoring.tex <==
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{Assets/Figures/Scoring.pdf}
%     \caption{Instruction tuning for scoring scenarios.}
%     \label{fig:scoring}
% \end{figure}

